Membership(s) and compliance(s) with class-based graphs

Besides the need for a better understanding of networks, there is a need for prescriptive models and tools to specify requirements concerning networks and their associated graph representations. We propose class-based graphs as a means to specify requirements concerning object-based graphs. Various variants of membership are proposed as special relations between class-based and object-based graphs at the local level, while various variants of compliance are proposed at the global level.

==> tikz_allNodes.tex <==
\newcommand{\NODExROMEO}{
	\node[object] (Romeo)
	{   \begin{tabular}{l} 	% content
		  \textbf{Romeo}\\
		  \hspace{0.2cm}{$\langle$name, Romeo$\rangle$}\\
		  \hspace{0.2cm}{$\langle$house, Montague$\rangle$}\\
      \hspace{0.2cm}{$\langle$sex, male$\rangle$}\\
		  \end{tabular}
 	};
}
